Distributed and Streaming Linear Programming in Low Dimensions

We study linear programming and general LP-type problems in several big data (streaming and distributed) models. We mainly focus on low dimensional problems in which the number of constraints is much larger than the number of variables. Low dimensional LP-type problems appear frequently in various machine learning tasks such as robust regression, support vector machines, and core vector machines. As supporting large-scale machine learning queries in database systems has become an important direction for database research, obtaining efficient algorithms for low dimensional LP-type problems on massive datasets is of great value. In this paper we give both upper and lower bounds for LP-type problems in distributed and streaming models. Our bounds are almost tight when the dimensionality of the problem is a fixed constant.

==> lbext.tex <==
\section{Lower bounds for high $d$}
In this section we claim the lower bounds for $d$-dimensional linear programming problem. By $\dLP$ we denote the communication problem when $n$ inequalities on $d$-dimensional vector $x$ are distributed among $k$ sites, and the goal is to compute the minimum value of the linear functional $f(x) = \sum\limits_{i = 1}^d c_i x_i$
which satisfies above inequalities.

Further we show that we cannot avoid the dependence on the dimension $d$ in communication protocols. At first we show that any protocol should spend at least $\Omega(kd)$ bits to solve the instance of $d$-dimensional linear programming. To obtain this bound we use the  straight-forward reduction of the Set Disjointness problem to the $d$-dimensional linear programming problem. 

In the Set Disjointness problem, $\Disj$, each site receives an input $X^i \in \set{0, 1}^n$, and the goal is to compute

\[\Disj_{n, k}(X^1, \dotsc, X^k) = \bigvee\limits_{j = 1}^n \bigwedge \limits_{i = 1}^k X^i_j\,.\]

The Set Disjointness problem is the hard problem and we cannot beat the trivial protocol. The following theorem reflects this fact.

\begin{theorem}[\cite{BEOPV13}]\label{thm:disj-lb}
	For every $\delta >0, n \geq 1$, and $k = \Omega(\log n)$ the communication complexity of the Set Disjointness problem is $\CC{\Disj_{n, k}} = \Omega(nk)$.
\end{theorem}

Using the above theorem we claim the lower bound on the $\dLP$.

\begin{theorem}
	For every $\delta > 0, n = \Omega(kd)$, and $k = \Omega(\log d)$ the communication complexity of $\dLP$ is $\CC{\dLP} = \Omega(dk)$.
\end{theorem}

\begin{proof}
	Consider the instance of $\Disj$ problem $X^1, \dotsc, X^k$ and show how to reduce the computation of the joint function $\Disj$ to solving $\dLP$. Because we assume that $f$ is shared information we can fix $f$ without communication and set one to the inner product with $d$-dimensional vector $c = (-1, \dotsc, -1)$. By using $X^i \in \set{0, 1}^d$ each site creates the following $d$ inequalities $x_1 \leq X^i_1, \dotsc, x_d \leq X^i_d$ (here we use $d$ instead $n$ in the Set Disjointness problem). Notice that the previous step can be done locally without communication.
	Because each inequalities involves only one variable we can claim that $\sum\limits_{i = 1}^d -x_i$ achieves the minimum value when $x_j = \min\limits_{i = 1}^k X^i_j$. Thus $\sum\limits_{j = 1}^{d}-x_j \leq -1$ if and only if 
	$\bigvee\limits_{j = 1}^d \bigwedge \limits_{i = 1}^k X^i_j = 1$. Thus we reduce the Set Disjointness on the ground set of $d$ elements to the $d$ dimensional linear programming. It is easy to see that the total number of inequalities in our reduction is bounded by $dk$. So on we can claim that for $n \geq dk$ the communication complexity of $d$ dimensional linear programming is at least the communication complexity of the Set Disjointness problem. In other words $\CC{\dLP} \geq \CC{\Disj_{d, k}} = \Omega(dk)$ (by Theorem~\ref{thm:disj-lb}) when $n \geq dk$. 
\end{proof}

The above result show that we cannot avoid the term $dk$ from the complexity even if we consider communication protocols with unbounded number of rounds.

In the next theorem we show that we cannot avoid from the term $d^{1-1/r} n^{1/r}$. To obtain this result we use the direct sum theorem for the two-party communication complexity from the work~\cite{JPY16}. From the high level we proved that a few instances of two-dimensional linear programs can be reduced to one instance of a fixed dimensional linear programming. So on by using the following direct sum argument we can claim the lower bound on fixed dimensional linear programming.

\begin{theorem}[\cite{JPY16}]\label{thm:directproduct}
	For any function $f$ and $k, r \leq 1$ the following fact is true that $\CCr{f^k}{r} = \Omega(\frac{k}{r}(\CCr{f}{r} - O(r^2)))$.
\end{theorem}

Here by $f^k$ we denote the communication problem of computing $k$ instances of the problem together.

Further we show how we can reduce the computation of $\frac{d}{2}$ instances of two dimensional linear programming problem to one $d$-dimensional linear programming problem and by Theorem~\ref{thm:directproduct} we claim that we cannot solve the resulted problem with communication significantly smaller than $d^{1-1/r} n ^{1/r}$.

\begin{theorem}
	$\CCr{\operatorname{LP}^{d, f}_{n, 2}}{r} = \Omega(\frac{d^{1 - 1/r}}{r}(n^{1/r}-r^2))$.
\end{theorem}


\begin{proof}
	We compress $m=\frac{d}{2}$ instances of $2$-dimensional linear programming on $\frac{n}{m}$ inequalities into one $d$-dimensional instance on $n$ inequalities in the following way.
	Consider $m$ instances of two-dimensional linear programming. The $i$-th problem depends on two variables $x_i, y_i$ and the objective function $f_0(x_i, y_i)$.
	Without loss of generality we can assume that for all $i$ the optimum value of $f_i$ is an integer number and lies inside the interval $[0, M)$ for a big integer number $M$. Actually, we never used the fact that coefficients of $f$ can be encoded in a small number of bits. Additionally, we assumed that $f$ is known as shared information, so we do not need to use the coefficients of $f$ during computations. We combine the set of functions into one super function of $d=2m$ variables 
	\[f(x_1, y_1, \dotsc, x_m, y_m) = \sum\limits_{i = 1}^m M^{i - 1} \times f_0(x_i, y_i)\,.\]
	
	As a set of inequalities each site of inequalities which one holds for $x_i, y_i$ because each pair of variables $x_i, y_i$ was restricted only by $\frac{n}{m}$ inequalities in total sites hold at most $n$ constraints for variables $x_1, y_1, \dotsc, x_m, y_m$. It is easy to see that if the set of feasible $(x_i, y_i)$ was $U_i \subset \mathbb R ^ 2$ then the set of feasible solutions of a new super problem is equal to $U_1 \times U_2 \times \dotsc \times U_m$. Thus we have that if $(x^*_i, y^*_i)$ is the optimal solution for $i$-th instance of $f_0$ then $(x^*_1, y^*_1, \dotsc, x^*_m, y^*_m)$ is the optimal solution for the new super problem. Because we assumed that value of each objective function is an integer number and bounded by $M$ if we compute the optimum value $f^*$ of $f$ we can easily reconstruct the value of each function $f_0(x_i^*, y_i^*)$. Especially, the optimum value of $i$-th instance of $f_0^*$ is equal to $i$-th digit of the number $f^*$ in $M$-base system. Thus we can claim that the communication complexity of $\CCr{\operatorname{LP}^{d, f}_{n, 2}}{r} \geq \CCr{\left(\operatorname{LP}^{2, f_0}_{2n/d, 2}\right)^m}{r} = \Omega(\frac{d^{1 - 1/r}}{r}(n^{1/r} - r^2))$.
\end{proof}
